Exploring prompts to elicit memorization in masked language model-based named entity recognition

Training data memorization in language models impacts model capability (generalization) and safety (privacy risk). This paper focuses on analyzing prompts' impact on detecting the memorization of 6 masked language model-based named entity recognition models. Specifically, we employ a diverse set of 400 automatically generated prompts, and a pairwise dataset where each pair consists of one person's name from the training set and another name out of the set. A prompt completed with a person's name serves as input for getting the model's confidence in predicting this name. Finally, the prompt performance of detecting model memorization is quantified by the percentage of name pairs for which the model has higher confidence for the name from the training set. We show that the performance of different prompts varies by as much as 16 percentage points on the same model, and prompt engineering further increases the gap. Moreover, our experiments demonstrate that prompt performance is model-dependent but does generalize across different name sets. A comprehensive analysis indicates how prompt performance is influenced by prompt properties, contained tokens, and the model's self-attention weights on the prompt.

==> introduction_mem.tex <==
\section{Introduction}


% Named Entity Recognition (NER) models \citep{rogers2020primer} have widespread applications in areas such as healthcare \citep{habibi2017deep}, social media \citep{yu-etal-2023-grounded}, and the justice system \citep{darji2023german}, where personally identifiable information such as person's names are commonly stored. The goal of NER tasks is to identify and label entities appearing in unstructured text into predefined categories \citep{nadeau2007survey}. Masked Language Models (MLMs), e.g., BERT \citep{devlin2019bert}, fine-tuned on various NER datasets achieve SOTA results \citep{nguyen2023auc, richie2023extracting, qu2023distantly}.

Fine-tuning Masked Language Models (MLMs), e.g., BERT \citep{devlin2019bert}, achieves SOTA results \citep{nguyen2023auc, richie2023extracting, qu2023distantly} on various ML tasks such as Named Entity Recognition (NER). However, recent studies have highlighted the memorization of training data in language models \citep{neel2023privacy}, especially for auto-regressive models such as GPT-2 \citep{mireshghallah2022empirical} and GPT-Neo \citep{carlini2023quantifying}, which expose them to extraction attacks \citep{carlini2021extracting} and membership inference attacks \citep{salem2018mlleaks} that can gather sensitive data from the models and lead to privacy risk. In contrast, few works explore the memorization issue of fine-tuned black-box MLMs (without access to model weights) toward privacy risk. 

\citet{tirumala2022memorization} use a metric the same as training accuracy to assess the memorization of MLMs toward learning ability. \citet{ali_unintended_2022} assume that a fine-tuned MLM memorizes a sample if the confidence of the samples In the Training data (In-train) is higher than all the samples Out of the Training data (Out-train), which can underestimate the privacy risk towards attacks that use a threshold \citep{mireshghallah_quantifying_2022}.  The above methods were originally designed to study memorization dynamics throughout the model training which relies on model weight changes and thus is not suitable for black-box models. \citet{carlini2021extracting} introduce extractability to measure the memorization of a black-box auto-regressive model. However, \citet{lehman-etal-2021-bert} failed to extract meaningful sensitive data from a fine-tuned black-box MLM. In this work, we fill up the need to design a new method for assessing the memorization of fine-tuned black-box MLMs toward privacy risk.
% \citet{lehman-etal-2021-bert} failed to extract the memorized sensitive data from a BERT model fine-tuned with a clinical dataset using a simple retrieve strategy. 

% Language models with memorization are vulnerable to membership inference attacks (MIAs) which aim to extract the training data from the models,  a successful MIA extracts sensitive training data of the NER models, violating the privacy of individuals involved in the training data \citep{jagannatha2021membership}. 

% The MIA proposed by \citet{salem2018mlleaks} assumes that machine learning models return a higher confidence score for data samples in the training data than for ones out of the training data. \citet{mireshghallah_quantifying_2022} and \citet{carlini2022membership} calculate a likelihood threshold to determine if a data sample belongs to the training data. The success of such MIAs exposes the extent of memorization by the model at the level of individual samples \citep{mireshghallah_quantifying_2022}. \citet{ali_unintended_2022} investigate the unintended memorization in the NER MLMs using a confidence-based MIA strategy and further demonstrate the unintended data memorization of NER MLMs. However, this category of MIAs relies heavily on the models' confidence scores, which can be sensitive to word changes of the input contents if the model is weak against adversarial attacks or badly calibrated \citep{feng-etal-2018-pathologies, jin2020bert}. Consequently, the success rate of MIAs is also affected by changes in the input. As no previous work has studied this hypothesis, we aim to close this research gap in this work.

% Previous works on MIA compute the success rate of attacks using a fixed prompt \citep{ali_unintended_2022}. Assuming that model confidence is sensitive to the input choice, that may lead to overestimation of the privacy risk of the NER model. Further, as we show in this paper, the attack success rates of prompts given different models---even if they share the same training data---are very weakly correlated. This means that rankings of model robustness can change drastically when a different attack prompt is used. Therefore, a reliable evaluation of model robustness to privacy attacks should include diverse attack prompts. To give recommendations on \textit{how} to diversify attack prompts, we explore which prompt properties most affect the attack success rate.

Our proposed method defines that an In-train sample is memorized by the model if the model gives a higher confidence score than an Out-train sample. Firstly, we create a new pairwise dataset composed of a large number of pairs of In-train and Out-train samples. Unlike \citep{ali_unintended_2022} that uses a single fixed prompt, i.e., My secret is XX, to retrieve confidence for a \textit{secret} entity from a NER model, our method considering the sensitivity of model confidence towards input changes \citep{jin2020bert} and thus exploring the impact of a set of 400 diverse prompts generated by an AI model (i.e., ChatGPT). The final memorization score for each prompt is measured by the percentage of the number of pairs that contain memorized samples in the dataset. 

We motivate our explorations with NER models fine-tuned on MLMs by their widespread applications in healthcare \citep{habibi2017deep}, social media \citep{yu-etal-2023-grounded}, and the justice system \citep{darji2023german}, where personally identifiable information such as person's names are commonly stored. The goal of NER tasks is to identify and label entities appearing in unstructured text into predefined categories \citep{nadeau2007survey}. Specifically, we investigate 6 NER models fine-tuned with CoNLL-2003 dataset \citep{tjong-kim-sang-de-meulder-2003-introduction}, the person's names (\textit{PER}) is considered as sensitive data \citep{lison2021anonymisation} in our study. Our pairwise dataset sampled from Wikidata \citep{vrandevcic2014wikidata} consists of a number of In-train $PER$ and an Out-train $PER$ pairs. A sentence integrated with a $PER$ and a prompt from the generated prompt set denoting the inputs to the MLM-base NER model for getting the confidence scores of the $PER$. Finally, we calculate memorization scores for different prompts over the pairwise dataset. Figure \ref{fig:framework} illustrated the full pipeline. Our contributions are: 

\begin{itemize}
    \item We are the first to propose a method to assess the memorization for fine-tuned black-box MLMs toward privacy risk with diverse prompts. We do not observe that memorization is affected by model size or architecture by exploring 6 black-box NER models with different model sizes and architectures.  
    
    \item We show that memorization assessment is sensitive to the prompt choice. The differences in memorization scores achieved by different prompts on the same model reached differences as large as 16\%. The score of the same prompt is model-dependent but generalized inside the dataset. 
  % \item We created a new pairwise dataset constructed with person's names from In-train data and Out-train data to estimate the memorization of NER models.  
    \item We apply the ensembling and prompt engineering techniques to the prompt set and observe that engineered (modified) prompts can improve 2\% upon the highest memorization score achieved by the original prompt set.
    % , but an ensemble of prompts does not bring additional improvement.
    
    \item We did a comprehensive analysis of how prompt properties affect the memorization scores at the sentence level and token level.
  
    
\end{itemize}


\begin{figure*}
  \centering
  \includegraphics[width=0.99\linewidth]{images/main.jpg}
  \caption{Memorization assessment of fine-tuned black-box MLMs. $P^{In}_*$ and $P^{Out}_*$ refer to a person's name in and out of the training data respectively.}
  \label{fig:framework}
\end{figure*}




==> introduction_mia.tex <==
\section{Introduction focus on MIA}

%1. Trying to explore privacy risks and propose ethical concerns
%2. How to relate to the search of the best prompt, [[attackers can actively do this]]

% The goal of the paper: we are not aiming at finding the best prompt. --> analysis paper

% How and why do attack prompts work?

% quantify the privacy risk of lm should also consider a wide range of attack prompts (not only a fix prompt), we examine several properties of the attack prompts and provide a clear guideline that one should use a diversity of attack prompts.

% why do not use generative models? mlm is more used in NER, check if there are the latest papers that use mlm for NER, so we can say that mlm is still advanced in NER.

% auto-aggressive models (prompt attack has been studied) and mlm

% find the most robust model with attack prompts across different properties.

% propose a metric to evaluate the robustness of the model --> 

% generalizable conclusions: attack prompt is generalizable; a recommendation on how to collect a valid set of attack prompts



% \textbf{— How can changing the input words influence the confidence score of model?}

% — How to get the best input words for achieving better ASR? (prompt tuning)

% \textbf{— How to best combine different prompts for achieving better ASR?}

% \textbf{— Training data memorization in BERT ner models. the larger model is more generalized?}

% \textbf{— Token-level analysis? why our method fails. Possible improvements can be made: only use the minimum token score of the name tokens.}

Named Entity Recognition (NER) models \citep{rogers2020primer} have widespread applications in areas such as healthcare \citep{habibi2017deep}, social media \citep{yu-etal-2023-grounded}, and the justice system \citep{darji2023german}, where personally identifiable information such as person's names are commonly stored. The goal of NER tasks is to identify and label entities appearing in unstructured text into predefined categories \citep{nadeau2007survey}. Masked Language Models (MLMs) fine-tuned on various NER datasets achieve SOTA results \citep{nguyen2023auc, richie2023extracting, qu2023distantly}.

However, recent studies have highlighted the privacy risks of MLMs when subjected to Membership Inference Attacks (MIAs) \citep{shokri2017membership}. Such attacks can successfully infer the membership of sensitive data to the training data of the NER models, violating the privacy of individuals involved in the training data \citep{jagannatha2021membership}.  

The MIA proposed by \citet{salem2018mlleaks} assumes that machine learning models return a higher confidence score for data samples in the training data than for ones out of the training data. \citet{mireshghallah_quantifying_2022} and \citet{carlini2022membership} calculate a likelihood threshold to determine if a data sample belongs to the training data. The success of such MIAs exposes the extent of memorization by the model at the level of individual samples \citep{mireshghallah_quantifying_2022}. \citet{ali_unintended_2022} investigate the unintended memorization in the NER MLMs using a confidence-based MIA strategy and further demonstrate the unintended data memorization of NER MLMs. However, this category of MIAs relies heavily on the models' confidence scores, which can be sensitive to word changes of the input contents if the model is weak against adversarial attacks or badly calibrated \citep{feng-etal-2018-pathologies, jin2020bert}. Consequently, the success rate of MIAs is also affected by changes in the input. 

Previous works on MIA compute the success rate of attacks using a fixed prompt \citep{ali_unintended_2022}. Assuming that model confidence is sensitive to the input choice, that may lead to over/under-estimation of the privacy risk of the NER model. Further, as we show in this paper, the attack success rates of prompts given different models---even if they share the same training data---are very weakly correlated. This means that rankings of model robustness can change drastically when a different attack prompt is used. Therefore, a reliable evaluation of model robustness to privacy attacks should include diverse attack prompts. To give recommendations on \textit{how} to diversify attack prompts, we explore which prompt properties most affect the attack success rate.


Specifically, we consider person's names (\textit{PER}) as sensitive data \citep{lison2021anonymisation} in our study. For the experiment, we first create a new pairwise attack dataset which is sampled from Wikidata \citep{vrandevcic2014wikidata} w.r.t the accessibility of a real-world attacker. The attack dataset is composed of a number of $PER$ pairs, with each pair containing a $PER$ from the training data of the NER models and a $PER$ out of training data. Then we use a generative AI model (ChatGPT\footnote{\url{https://chat.openai.com}}) to generate 400 different sentences as the attack prompts. The integrated sentences of the $PER$ from the attack dataset and attack prompts denote to the inputs to NER MLMs for getting the confidence scores of the $PER$. In the end, a successful MIA is achieved if the confidence score of the $PER$ in the training data is higher than the $PER$ out of the training data, otherwise, the attack failed. The attack success rate (ASR = $\#\textit{successful attacks}/\#\textit{attempted attacks}$) is used to evaluate the privacy risk of the attacked NER model. Figure \ref{fig:framework} illustrated the full pipeline.


Contribution: 
% todo: need more thinking and quantifying
\begin{itemize}
    \item We build a pipeline to evaluate the robustness of privacy risks of NER MLMs toward a set of attack prompts with a new proposed metric. 
  \item  We showed that We show that the attack success rate varies depending on the attack prompt, reaching differences as large as 16 percentage points. The performance of the same attack prompt is model-dependent. 
  \item We created a new pairwise attack dataset constructed with person's names from In-train data and Out-of-train data to estimate the privacy risk of NER models.  
    \item We found that \textit{ASR} of an attack prompt does not generalize across models: an attack prompt that successfully attacks a model may be ineffective for another one. Conversely, the ASR of an attack prompt  \textit{does} generalize from the development to the test split.
    
    \item We did a comprehensive analysis of how prompt properties affect the success rates of attacks considering different models.
  
    
\end{itemize}







% — Against differential privacy training methods to find a tradeoff of methods.

% -- Each prompt is a labeling function
% -- flying squid to weight (additional functions)
% -- Collaboration of answers confidence
% -- instruction prompting tuning to get the confidence model.
% -- 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

